HyperMono: A Monotonicity-aware Approach to Hyper-Relational Knowledge Representation

In a hyper-relational knowledge graph (HKG), each fact is composed of a main triple associated with attribute-value qualifiers, which express additional factual knowledge. The hyper-relational knowledge graph completion (HKGC) task aims at inferring plausible missing links in a HKG. Most existing approaches to HKGC focus on enhancing the communication between qualifier pairs and main triples, while overlooking two important properties that emerge from the monotonicity of the hyper-relational graphs representation regime. Stage Reasoning allows for a two-step reasoning process, facilitating the integration of coarse-grained inference results derived solely from main triples and fine-grained inference results obtained from hyper-relational facts with qualifiers. In the initial stage, coarse-grained results provide an upper bound for correct predictions, which are subsequently refined in the fine-grained step. More generally, Qualifier Monotonicity implies that by attaching more qualifier pairs to a main triple, we may only narrow down the answer set, but never enlarge it. This paper proposes the HyperMono model for hyper-relational knowledge graph completion, which realizes stage reasoning and qualifier monotonicity. To implement qualifier monotonicity HyperMono resorts to cone embeddings. Experiments on three real-world datasets with three different scenario conditions demonstrate the strong performance of HyperMono when compared to the SoTA.

==> sections/summary_of_changes.tex <==
% \noindent{\bf \large \textcolor{blue}{Meta Reviewer}}

% \noindent \textbf{Q1: Clear rationale behind the performance improvement.} \textbf{A:} Firstly, we have formally proved that cones faithfully encode the qualifier monotonicity in \shzw{\textbf{{\textbf{\hyperlink{proof_of_propositions}{Appendix. I}}}}}. Secondly,  ShrinkE~\citep{Bo_2023} uses box embeddings to encode  the  qualifier monotonicity. However, the offsets of boxes are unbounded, which brings uncertainty to the box embedding, while the angle and aperture of cone embedding are limited [$-\pi$, $\pi$) and [0, $2\pi$], ensuring the boundedness of the cone operation. In addition, we have strengthened the content about qualifier monotonicity from multiple perspectives, including dataset construction, methods, and experimental analysis.

% \noindent \textbf{Q2: Clarify the details of the experimental environments.}  \textbf{A:} We have provided all the running logs in the anonymous open source code (see: \shzw{\textbf{\url{https://anonymous.4open.science/r/HKGC-HyperMono-AE61}}}). In addition, we have also added more details about experimental environment  in \shzw{\textbf{\hyperlink{protocol_and_implements}{Appendix C}}}.

% \smallskip
% %\section*
% \noindent{\bf \large \textcolor{blue}{Reviewer 1avR}}


% \noindent \textbf{Q1: The model's complexity.} 

% \noindent \textbf{A:} We have added complexity analysis in \shzw{\textbf{\hyperlink{complexity_analysis}{Appendix E}}}, including: a) \textit{time complexity}; b) \textit{space complexity}; c) \textit{model training time}; d) \textit{inference time per sample}; and e) \textit{GPU memory consumption}.

% \noindent \textbf{Q2: The limited diversity in hyper-relational knowledge.}

% \noindent \textbf{A:} Originally, to ensure the fairness of the experimental comparison, we selected the benchmarks that are consistent with baselines. %Enriching the hyper-relational knowledge alone will lead to unfair experimental comparison. 
% However, the subsets results in \shzw{\textbf{Table~\ref{table_fixed_percentage_fixed_qualifier}}} and \shzw{\textbf{Table~\ref{table_fixed_percentage_mixed_qualifier}}} are actually experiments on different hyper-relational knowledge richness.

% \noindent \textbf{Q3: The experiments in other environments.}

% \noindent \textbf{A:} We have added a number of additional experiments, including: \textit{different of neighbor numbers} and \textit{different of sparsity ratio}, the corresponding results and analysis can be found in \shzw{\textbf{\hyperlink{additional_results}{Appendix F}}}.


% We have added a number of additional experiments, including: a) \textit{different of pooling operation}; b) \textit{different of aggregation operation}; c) \textit{different of embedding space}; d) \textit{different of learning rate}; e) \textit{different of neighbor numbers}; and f) \textit{different of sparse ratio}, the corresponding results and analysis can be found in \shzw{\textbf{\hyperlink{additional_results}{Appendix F}}}.

\smallskip
%\section*
\noindent {\large \bf \textcolor{blue}{Reviewer VZN3}}


\noindent \textbf{Q1: \texttt{HyperMono}'s performance improvement.}

\noindent \textbf{A:} In \shzw{\textbf{Table~\ref{table_mixed_percentage_mixed_qualifier}}}, we have added the experimental results of predicting all entities at different positions. We find that compared with predicting only \textit{Head/Tail}, \texttt{HyperMono} has a greater performance advantage in predicting \textit{All Entities}. %In the subsequent \shzw{\textbf{Table~\ref{table_fixed_percentage_fixed_qualifier}}} and \shzw{\textbf{Table~\ref{table_fixed_percentage_mixed_qualifier}}}, we focus on the more challenging task of predicting 
Regarding the \textit{Head/Tail} setting, we have also added the possible reasons for the small improvement in the experimental analysis.

\noindent \textbf{Q2: Predicting all entities in hyper-relational facts.}

\noindent \textbf{A:} We have added the task definitions in \shzw{\textbf{Section~\ref{section_preliminaries}}}: \textit{Head/Tail} and \textit{All Entities}, where \textit{Head/Tail} is the original task  on and \textit{All Entities} is the task you proposed. Results can be found in \shzw{\textbf{Table~\ref{table_mixed_percentage_mixed_qualifier}}}.

\noindent \textbf{Q3: Technical analysis of the proposed method.}

\noindent \textbf{A:} Please see the response to Meta Reviewer's \shzw{\textbf{Q1}}.

\smallskip
%\section*
\noindent {\bf\large  \textcolor{blue}{Reviewer Uapj}}

\noindent \textbf{Q1: How does the dataset satisfy the qualifier monotonicity.}

\noindent \textbf{A:} We have added the dataset construction description in \shzw{\textbf{\hyperlink{datasets}{Appendix A}}}, including \textit{from nothing to something} and \textit{from little to more}, which  ensure the qualifier monotonicity of the entire dataset.


%\section*

\smallskip
\noindent{\large \bf \textcolor{blue}{Reviewer DdUU}}

\noindent \textbf{Q1: Running example.}

\noindent \textbf{A:} Using the example in \shzw{\textbf{Figure~\ref{figure_instance}}}, we have strengthened the motivation in  \shzw{\textbf{Section~\ref{introduction}}}. In addition, we have also added a Case Study in \shzw{\textbf{\hyperlink{case_study}{Appendix H}}}.

\noindent \textbf{Q2: Analyzing effectiveness, efficiency, and memory usage.}

\noindent \textbf{A:} Regarding effectiveness, we have tested it in different scenarios in \shzw{\textbf{Tables~\ref{table_mixed_percentage_mixed_qualifier}}}, \shzw{\textbf{~\ref{table_fixed_percentage_fixed_qualifier}}}, and \shzw{\textbf{~\ref{table_fixed_percentage_mixed_qualifier}}}. Regarding effectiveness and memory usage, we have explained it separately in \shzw{\textbf{\hyperlink{complexity_analysis}{Appendix E}}}.

\noindent \textbf{Q3: Technical analysis of the proposed method.}

\noindent \textbf{A:} Please see the response to Meta Reviewer's \shzw{\textbf{Q1}}.

\noindent \textbf{Q4: Different alternative approaches in each step.}

\noindent \textbf{A:} We have added a number of additional experiments, including: \textit{different of pooling operation}, \textit{different of aggregation operation} and \textit{different of embedding spaces}. The corresponding results and analysis can be found in \shzw{\textbf{\hyperlink{additional_results}{Appendix F}}}.

\noindent \textbf{Q5: Improve the plot quality.}

\noindent \textbf{A:} We have bolded the lines in \shzw{\textbf{Figure~\ref{figure_hyper_parameters}}}.

\smallskip
%\section*
\noindent{\large \bf \textcolor{blue}{Reviewer YVb3}}

\noindent \textbf{Q1: $\beta_{\mathcal{S}_i}$ is smaller than $\beta_{h,r}$.}

\noindent \textbf{A:} We have corrected the minor error in \shzw{\textbf{Equation~\ref{equation_3}}}.

\noindent \textbf{Q2: The existence of $C_S$.}

\noindent \textbf{A:} We have added an explanation of the existence of $C_S$ in the \textit{Cone Shrinking} part in \shzw{\textbf{Section~\ref{sec:MEP}}}.

\noindent \textbf{Q3: Replace QMP with a simple transform.}

\noindent \textbf{A:} We have added the results of replacing the \texttt{QMP} operation with the simpler \texttt{TP} operation in the \texttt{None} row of \shzw{\textbf{Table~\ref{table_additional_results}}}. In addition, we have also added the results of replacing cone with \texttt{Beta} and \texttt{Gamma} embeddings in \shzw{\textbf{Table~\ref{table_additional_results}}}.

\noindent \textbf{Q4: Case study.}
\textbf{A:} We have added a Case Study in \shzw{\textbf{\hyperlink{case_study}{Appendix H}}}.

\noindent \textbf{Q5: The relations between HKGC and KHC.}

\noindent \textbf{A:} We have provided a more detailed and explicit definition of the HKGC task in \shzw{\textbf{Section~\ref{section_preliminaries}}}, which includes predicting \textit{Head/Tail} entities and \textit{All Entities}. We have also presented a comparison of different models in \shzw{\textbf{Table~\ref{table_mixed_percentage_mixed_qualifier}}}. Moreover, the previously studied \textit{knowledge hypergraph completion} (\textit{knowledge hypergraph link prediction}) is a different task from HKGC, as evidenced by the selection of baselines. However, by adopting the data processing approach of PolygonE~\cite{Shiyao_2022}, we can unify both tasks. So we have conducted an evaluation of \texttt{HyperMono}’s capability in knowledge hypergraph link prediction in \shzw{\textbf{\hyperlink{model_transferability}{Appendix G}}}.  Note that this evaluation is merely to test \texttt{HyperMono}’s transferability and is not our core focus.

\noindent \textbf{Q6: About \texttt{HyperMono}'s reproducibility.}

\noindent \textbf{A:} Our results are fully reproducible, and we have provide all run logs in the anonymous open source code repository (see \shzw{\textbf{Abstract}} part). In addition, we have also added more details about the experimental environment in \shzw{\textbf{\hyperlink{protocol_and_implements}{Appendix C}}}.

%\section*
\smallskip 
\noindent {\large \bf \textcolor{blue}{Reviewer BywK}}

\noindent \textbf{Q1: More detailed model implementation details.}

\noindent \textbf{A:} Please see answer to \shzw{\textbf{Q6}} of reviewer \shzw{\textbf{YVb3}} above.

%We have provide all run logs in the anonymous open source code repository and added more descriptions about the experimental environment in \shzw{\textbf{\hyperlink{protocol_and_implements}{Appendix C}}}.

\noindent \textbf{Q2: Additional ablation experiments.}

\noindent \textbf{A:} We have %further conducted incremental experiments and added corresponding experimental analysis 
added them in \shzw{\textbf{\hyperlink{additional_results}{Appendix F}}}.

\noindent \textbf{Q3: Experimental results for other edge cases.}

\noindent \textbf{A:} In the \textit{effect of sparse ratio} of \shzw{\textbf{\hyperlink{additional_results}{Appendix F}}}, we have performed more extreme boundary condition tests (\textit{i.e.,} testing the performance of the model when less neighbor information is available).

\noindent \textbf{Q4: Comparison with broader baselines.}

\noindent \textbf{A:} We have added the latest literature results in the HKGC field HyperCL~\citep{Yuhuan_2024} in \shzw{\textbf{Table~\ref{table_mixed_percentage_mixed_qualifier}}}, \shzw{\textbf{Table~\ref{table_fixed_percentage_fixed_qualifier}}}, and \shzw{\textbf{Table~\ref{table_fixed_percentage_mixed_qualifier}}}.

\noindent \textbf{Q5: Clarify mathematical equations.}

\noindent \textbf{A:} We have explained the notation and functionality  of \shzw{\textbf{Equation~\ref{equation_2}}} and \shzw{\textbf{Equation~\ref{equation_3}}} in more detail.
